Spectral Norm of Convolutional Layers with Circular and Zero Paddings

This paper leverages the use of \emph{Gram iteration} an efficient, deterministic, and differentiable method for computing spectral norm with an upper bound guarantee. Designed for circular convolutional layers, we generalize the use of the Gram iteration to zero padding convolutional layers and prove its quadratic convergence. We also provide theorems for bridging the gap between circular and zero padding convolution's spectral norm. We design a \emph{spectral rescaling} that can be used as a competitive $1$-Lipschitz layer that enhances network robustness. Demonstrated through experiments, our method outperforms state-of-the-art techniques in precision, computational cost, and scalability. The code of experiments is available at https://github.com/blaisedelattre/lip4conv.

==> sections/archive.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Weight decay strided case}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Aliasing}
% \blaise{draft}
% From wikipedia : 
% with $x(t)$ a function with a Fourier transform $X(f)$.

% \begin{thm} (Shannon)
% If a function 
% x(t) contains no frequencies higher than $b$ hertz, then it can be completely determined from its ordinates at a sequence of points spaced less than $\frac{1}{2b}$ seconds apart.
% \end{thm}

% Equivalently, for a given sample rate $f_{s}$, perfect reconstruction is guaranteed possible for a band limit $b < \frac{f_s}{2}$.

% \paragraph{Shannon original proof flavor}

% $f_s = 2b$

% $X(f)= \int_{-\infty}^{\infty} x(t) e^{- \ci 2 \pi f t} dt$. \\
% $x(t) = \frac{1}{2\pi}\int_{-\infty}^{\infty} X(w) e^{\ci 2 \pi w t} dw = \frac{1}{2\pi}\int_{-2\pi b}^{2\pi b} X(w) e^{\ci 2 \pi w t} dw $

% because $X(w) = 0$ for $|\frac{w}{2 \pi}| < b$.

% if we let $t=\frac{k}{2b}$, where $k \in \mathbb{Z}$,

% $$x \left( \frac{k}{2b} \right) = \frac{1}{2\pi}\int_{-2\pi b}^{+2\pi b} X(w) e^{ \ci \frac{1}{2b} k w } dw$$
% "this determines Fourier coefficient of $X(w)$, and then determines $X(w)$, and thus determines $x(t)$ completely."

% Cela signifie que si $x$ est périodique avec une période de $\frac{1}{2b}$, alors $x$ est déterminé par des fréquences $f < 2b$ et que le signal peut être bien reconstitué par des coefficients de Fourier de fréquences $f < 2b$. Autrement non, et cela produit des artefacts : repliement spectral.


% Here we have an input  $x$   and we subsample with stride/period $g > 1$. We recognize $2b = \frac{1}{g}$, so max frequency of signal must be below $b =  \frac{1}{2g}$. For a signal being a discrete sequence of $n$ points $x \in \mathbb{R}^n$, 


% \paragraph{Density of g-Toeplitz}
% \cite{yi2020asymptotic}
% For a stride size $g > 1$, the matrix representing the strided convolution product $T^g \in \mathbb{R}^{\cout n^2 / g^2 \times \cin n^2}$ becomes a block g-Toeplitz matrix. We consider the same stride in both directions. \\
% $T^g = (T_{gk_1})_{k_1=1}^{n/g}$, 
% where $T_{gk_1} = (T_{gk_1, gk_2})_{k_2=1}^{n/g}$, with $T_{gk_1, gk_2} = K_{:, :, gk_1, gk_2}^\Uparrow \in \mathbb{R}^{\cout \times \cin}$.

% From \cite{ngondiep_spectral_2010}, 
% the spectral density matrix of $T^g$ writes as :

% $E(w_1, w_2) = \sqrt{\frac{1}{g^2} \sum_{m_1= 0}^{g-1} \sum_{m_2 = 0}^{g-1} f^2(w_1, w_2, m_1, m_2)}$

% $f(w_1, w_2, m_1, m_2) = \sum_{k_1 = 1}^k \sum_{k_2 = 1}^k T_{gk_1, gk_2} e^{\ci \frac{1}{g} (k_1 (w_1+2\pi m_1) + k_2 (w_2+2\pi m_2))}$ \\

% Let $ 1 \leq k_1^\prime, k_2^\prime \leq k/g$,
% $$T^g_{k_1^\prime, k_2^\prime} = T_{gk_1, gk_2} = \frac{1}{(2 \pi)^2} \int_{-\pi}^\pi \int_{-\pi}^\pi E(w_1, w_2) e^{-\ci \frac{1}{g} (k_1 w_1 + k_2 w_2)} dw_1 dw_2$$

% \blaise{check}

% Here we considered an already discrete signal that we downsample with frequency $\frac{1}{g}$.

% Gaussian filter for $2$-dimensional signal $x$
% \begin{align*}
% y(i, j) &= \int_{-\infty}^{\infty} \int_{-\infty}^{\infty} x(u, v) \cdot G_\sigma(i - u, j - v) \, du \, dv \\
% &= \int_{-\infty}^{\infty} \int_{-\infty}^{\infty} x(u, v) \cdot \frac{1}{(2 \pi \sigma^2)^{1/2}} \exp \left( -\frac{(i - u)^2 + (j - v)^2}{2 \sigma^2} \right) \, du \, dv \\
% &= \frac{1}{(2 \pi \sigma^2)^{1/2}} \int_{-\infty}^{\infty} \int_{-\infty}^{\infty} x(u, v) \cdot \exp \left( -\frac{(i - u)^2 + (j - v)^2}{2 \sigma^2} \right) \, du \, dv
% \end{align*}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Autres idées pour généraliser}

% \section{Idées / Pistes}
% \begin{itemize}
%     \item quelle relation entre $\sigma_1(C^\Uparrow)$ et $\sigma_1(T^\Uparrow)$ ?
%     \item étendre preuves avec stride dans matrice circulante/Toeplitz
%     \item étendre preuves du zero padding au constant padding (non-zero padding)
%     \item Zhang2019: circular convolution, shift-equivariance, shift invariance. true for zero-padded conv?
%     \item sampling hautes basses frequences de la densité de spectral density matrix, générer des conv hautes ou basses frequences
%     \item Différence circular vs padded ConvNets: on accuracies and training times
% \end{itemize}


\subsection{Common bound on circulant and Toeplitz matrix without Fourier transform}
\blaise{Work in progress here}
We can write
\begin{align*}
    &\max_{1 \leq u,v \leq n} \norm{D_{u,v}^{(t)}}_F^2 
     \leq \max_{w_1, w_2 \in [0, 2\pi]} \norm{E(w_1,w_2)^{(t)}}_F^2\\ 
     %
     &= \max_{w_1,w_2 \in [0, 2\pi]} \norm{
      \left( \sum_{k_1=0}^{k-1} \sum_{k_2=0}^{k-1} 
     e^{-\frac{2\pi\ci k_1 w_1}{n}} e^{-\frac{2\pi\ci k_2 w_2}{n}}  K_{:,:,k_1, k_2} \right)^{(t)}}_F^2 \\
     %
     &= \max_{w_1,w_2 \in [0, 2\pi]} \sum_{j=1}^{\cout} \sum_{i=1}^{\cin} \left | 
     \left( \sum_{k_1=0}^{k-1} \sum_{k_2=0}^{k-1} 
     e^{-\frac{2\pi\ci k_1 w_1}{n}} e^{-\frac{2\pi\ci k_2 w_2}{n}}  K_{:,:,k_1, k_2} \right)_{i,j}^{(t)}
     \right |^2 \\
     %
     &= \max_{w_1,w_2 \in  [0, 2\pi]} \sum_{j=1}^{\cout} \sum_{i=1}^{\cin} 
     \left( 
        \sum_{k_1=0}^{k-1} \sum_{k_2=0}^{k-1} 
        e^{-\frac{2\pi\ci k_1 w_1}{n}} e^{-\frac{2\pi\ci k_2 w_2}{n}}  K_{:,:,k_1, k_2}
        \sum_{k_1^\prime=0}^{k-1} \sum_{k_2^\prime=0}^{k-1} 
        e^{\frac{2\pi\ci k_1^\prime w_1}{n}} e^{\frac{2\pi\ci k_2^\prime w_2}{n}}  K_{:,:,k_1^\prime, k_2^\prime}^\top
     \right)_{i,j}^{2^{t-1}}
     \\
     %
     &= \max_{w_1,w_2 \in [0, 2\pi]} \sum_{j=1}^{\cout} \sum_{i=1}^{\cin} 
     \left( 
        \sum_{k_1=0}^{k-1} \sum_{k_2=0}^{k-1} 
        \sum_{k_1^\prime=0}^{k-1} \sum_{k_2^\prime=0}^{k-1}
        e^{\frac{2\pi\ci (k_1^\prime-k_1) w_1}{n}} e^{\frac{2\pi\ci (k_2^\prime-k_2) w_2}{n}}  
        K_{:,:,k_1, k_2}
        K_{:,:,k_1^\prime, k_2^\prime}^\top
     \right)_{i,j}^{2^{t-1}}
     \\
\end{align*}
We call the $t^{th}$ Gram iterate $K_{:,:,k_1, k_2}^{(t)}$ of matrix $K_{:,:,k_1, k_2}$ of size $\cout \times \cin$. Using inequality between arithmetic and quadratic mean we get :

\begin{align*}
\max_{1 \leq u,v \leq n} \norm{D_{u,v}^{(t)}}_F^2 &\leq k^{2^t}  \sum_{j=1}^{\cout} \sum_{i=1}^{\cin}  
\sum_{k_1=0}^{k-1} \sum_{k_2=0}^{k-1} 
\left | K_{i,j,k_1, k_2}^{(t)} \right|^2 \\
%
\max_{1 \leq u,v \leq n} \norm{D_{u,v}^{(t)}}_F^{2^{1-t}} &\leq k
\left(
\sum_{j=1}^{\cout} \sum_{i=1}^{\cin}  
\sum_{k_1=0}^{k-1} \sum_{k_2=0}^{k-1} 
\left | K_{i,j,k_1, k_2}^{(t)} \right|^2
\right)^{2^{-t}} \ .
\end{align*}


\newpage
\section{Rescale}

\begin{algorithm}[h]
\caption{: Lip\_dense$(G, N_\text{iter})$}
\label{algo:gram_iteration_dense}
\begin{algorithmic}[1]
  \STATE \textbf{Inputs} matrix: $G$, number of iterations: $N_\text{iter}$
  \STATE  $r \gets 0$ \hfill \text{// initialize rescaling}
  \STATE \textbf{for} $1 \ldots N_\text{iter}$
    \STATE \quad $G \gets G/\norm{G}_F$ \hfill \text{// rescale to avoid overflow}
    \STATE \quad $G \gets G^* G$ \hfill \text{// Gram iteration}
    \STATE  \quad $r \gets 2(r + \log \norm{G}_F)$ \hfill \text{// cumulate rescaling}
  \STATE $\sigma_1 \gets \norm{G}_F^{2^{-N_\text{iter}}} \exp{(2^{-N_\text{iter}} r})$
  \STATE \textbf{return} $\sigma_1$
\end{algorithmic}
\end{algorithm}

Example for $N_{iter}=1$
\begin{align*}
    &G_1 = G^* G / \norm{G}_F^2 \\
    &r_1 = 2(0 + \log \norm{G_1}_F) =  2 \log \norm{G_1}_F\\
    &\sigma_1 = \norm{G_1}_F^{2^{-1}} \exp{(2^{-1} r_1)} \\
    &\sigma_1 = \norm{G^* G / \norm{G}_F^2}_F^{1/2} \exp{(\frac{1}{2} 2 \log \norm{G^* G / \norm{G}_F^2}_F)} \\
    &\sigma_1 = \norm{G^* G }_F^{1/2}/ \norm{G}_F \exp{(\log \norm{G^* G / \norm{G}_F^2}_F)} \\
\end{align*}

Example for $N_{iter}=1$ bis
\begin{align*}
    &G_1 = G^* G / \norm{G}_F^2 \\
    &r_1 = 2(0 + \log \norm{G}_F) =  2 \log \norm{G}_F\\
    &\sigma_1 = \norm{G^* G / \norm{G}_F^2}_F^{2^{-1}} \exp{(2^{-1} r_1)} \\
    &\sigma_1 = \norm{G_1}_F^{2^{-1}} \exp{(2^{-1} 2 \log \norm{G}_F)} \\
    &\sigma_1 = \norm{G^* G }_F^{2^{-1}}  \norm{G}_F / \norm{G}_F \\
    &\sigma_1 = \norm{G^* G }_F^{2^{-1}} \\
\end{align*}


Example for $N_{iter}=2$
\begin{align*}
    &G_1 = G^* G / \norm{G}_F^2 \\
    &r_1 = 2(0 + \log \norm{G_1}_F) =  2 \log \norm{G_1}_F\\
    &G_2 = G_1^* G_1 / \norm{G_1}_F^2 \\
    &r_2 = 2(2\log \norm{G_1}_F + \log \norm{G_2}_F)  \\
    &r_2 = 4\log \norm{G_1}_F + 2\log \norm{G_2}_F)  \\
    &\sigma_1 = \norm{G_2}_F^{2^{-2}} \exp{(2^{-2} r_2)} \\
    &\sigma_1 = \norm{G_1^* G_1 / \norm{G_1}_F^2}_F^{1/4} \exp{(1/4 \log \norm{G_1}_F + 1/2\log \norm{G_2}_F)} \\
    &\sigma_1 = \norm{G_1^* G_1 / \norm{G_1}_F^2}_F^{1/4} \exp{(1/4 \log \norm{G_1}_F + 1/2\log \norm{G_1^* G_1 / \norm{G_1}_F^2}_F)} \\
\end{align*}


% \blaise{En fait c'est pas le meilleur des deux entre rescaling et spectral normalization, c'est une "interpollation", faible iter : régime rescaling. bcp d'iter : régime spectral normalization. \\
% Le rescaling est assez grossier avec $n_{iter}=1$ (AOL regime) mais pendant l'entrainement l'optim fait que les layers sont intéressantes, en rescaling pures je suis pas convaincu vu que la borne sur la spectral norm est tres grossière. Je vais prendre les spectrum des convolutions apres entrainement pour l'exp. En tout cas je pense que le message est pas exactement celui dont on avait discuté.}


==> sections/frobenius_draft.tex <==
\section{Frobenius norm of convolutional layers and Weight decay}
We recall the expression of the Frobenius norm for a matrix $W$ :
\begin{align*}
  \norm{W}_F = \left( \sum_{i=1}^{\min\{p, q\}} \sigma_i^2(W) \right)^{1/2} \geq \sigma_1(W) = \norm{W}_2 \ .  
\end{align*}
How is this norm written for the convolutional layer?

\subsection{Circular convolution}

The Frobenius norm on the layer is defined as the Frobenius norm of the matrix $C$ describing the operator.

\begin{prop}
\label{prop:circular_conv_frob}
For a circular convolutional layer $C$ parametrized by a filter $K \in \mathbb{R}^{\cout \times \cin \times k \times k}$, and for an input $X \in \mathbb{R}^{\cin \times n \times n }$, we have:
\begin{align}
    \norm{C}_F = n \norm{K}_F \ .
\end{align}
\end{prop}


\subsection{Toeplitz convolution}

For the Toeplitz convolutional layer, we can count the number of times an element of the kernel $K$ is hoovered over a pixel of the image.
\begin{prop}
For a Toeplitz convolutional layer $T$ parametrized by a filter $K \in \mathbb{R}^{\cout \times \cin \times k \times k}$, and for an input $X \in \mathbb{R}^{\cin \times n \times n }$, we have:
\begin{align}
    \norm{T}_F = \left\lfloor\frac{n + 2 \text{padding}- k -1}{\text{stride}} +1 \right \rfloor \norm{K}_F \ .
\end{align}
\end{prop}

\subsection{Weight decay of convolutional layers}

Weight decay regularizes the squared Frobenius norm of weights to avoid overfitting, in the case of dense layers it is equivalent to regularizing the Frobenius norm of the weight matrix $W$ which is the sum of all singular values.
%
Weight decay for a convolution is performed by regularizing $\norm{K}_F$ which is not equivalent to regularizing the sum of singular values of $T$ or $C$.

For dense layers, regularizing the matrix $W$ or its parameters is the same, for convolutional layers, it is not the same.
Let us consider a convolutional layer and the associated circulant or Toeplitz matrix $W \in \{ C, T \}$ constructed with filter $K$ and input size $n$.
However, applying weight decay on convolutional layer parameters $K$ is going to regularize $\norm{K}_F = \frac{\norm{W}_F}{n}$ this corresponds to a lower regularization to layers where input spatial size $n$ is large for the same $\norm{K}_F$.
For a ResNet152 on ImageNet, the starting input spatial size is $n=224$ and the lower spatial size for features is $7$, w.r.t to Frobenius norm of $W$ the last convolutional layers can be regularized up to $32$ times what first convolutional layers are being regularized.
A correction can be applied to weight decay to take into account this effect and regularize the Frobenius norm effectively. Similar corrections were applied in AdamW to weight decay when it was modified by optimizer rescale \citep{loshchilov2017decoupled}.


\subsection{Proof of \ref{prop:circular_conv_frob}}
\begin{prop*}
For a circular convolutional layer $C$ parametrized by a filter $K \in \mathbb{R}^{\cout \times \cin \times k \times k}$, and for an input $X \in \mathbb{R}^{\cin \times n \times n }$, we have:
\begin{align}
    \norm{C}_F = n \norm{K}_F \ .
\end{align}
\end{prop*}
\begin{proof}
For circular padding convolution using Theorem~\ref{theorem:block_diagonalization}, $C$ can be block diagonalized with blocks $D_i$.
The squared Frobenius norm of $C$ is then the sum of the squared  Frobenius norm of the $D_{u,v}$ :
    \begin{align*}
    \norm{C}_F^2 &= \sum_{u=1}^{n}\sum_{v=1}^{n} \norm{D_{u,v}}_F^2 \\
    &= \sum_{u=1}^{n}\sum_{v=1}^{n} 
        \sum_{i=1}^{\cout}\sum_{j=1}^{\cin} D_{u,v, i, j}^2 \\
    &= \sum_{i=1}^{\cout}\sum_{j=1}^{\cin} \norm{D_{:,:,i,j}}^2_F \\
    &= \sum_{i=1}^{\cout}\sum_{j=1}^{\cin} \norm{U^T K_{i,j,:,:} U}^2_F \\
    &=  n^2 \sum_{i=1}^{\cout}\sum_{j=1}^{\cin} K_{i,j,:,:}^2 \\
    &= n^2 \norm{K}_F^2 \ .
\end{align*}
\end{proof}

